Are We There Yet? Unraveling the State-of-the-Art Graph Network Intrusion Detection Systems

Network Intrusion Detection Systems (NIDS) are vital for ensuring enterprise security. Recently, Graph-based NIDS (GIDS) have attracted considerable attention because of their capability to effectively capture the complex relationships within the graph structures of data communications. Despite their promise, the reproducibility and replicability of these GIDS remain largely unexplored, posing challenges for developing reliable and robust detection systems. This study bridges this gap by designing a systematic approach to evaluate state-of-the-art GIDS, which includes critically assessing, extending, and clarifying the findings of these systems. We further assess the robustness of GIDS under adversarial attacks. Evaluations were conducted on three public datasets as well as a newly collected large-scale enterprise dataset. Our findings reveal significant performance discrepancies, highlighting challenges related to dataset scale, model inputs, and implementation settings. We demonstrate difficulties in reproducing and replicating results, particularly concerning false positive rates and robustness against adversarial attacks. This work provides valuable insights and recommendations for future research, emphasizing the importance of rigorous reproduction and replication studies in developing robust and generalizable GIDS solutions.

==> tex/Acknowledgments.tex <==
\section{Acknowledgments}

==> tex/background.tex <==
\subsection{Background: \gnids}
\begin{comment}
\pj{
The Intrusion Detection System (IDS) plays an important role in enterprise security infrastructure, which continuously
monitors and analyzes computer systems or networks to detect malicious activities \cite{zhong2024survey}. Depending on the source of data, Intrusion Detection Systems can be categorized into host-based IDS(HIDS) and network-based IDS(NIDS) \cite{debar1999towards}. HIDS detects anomalies at the operating system level or within specific applications running on a single host. NIDS, on the other hand, monitor network traffic to detect suspicious patterns or activities. In this paper we focus on NIDS, which captures and analyzes packets flowing through the network.}

\pj{The effectiveness of NIDS is often determined by their detection methods. Traditional NIDS based on detection rules matching are effective against known threats~\cite{zeek, suricata, snort, modSecurity, yara}. However, they struggle to detect unknown attack patterns, which leads to high false negative rates. To address this problem, \gnids have been developed by integrating graph learning techniques with intrusion detection systems.}

\pj{Graph is a fundamental concept in mathematics and computer science used to represent relationships between objects. A graph $\mathcal{G}$ can be defined as an ordered pair 
$\mathcal{G} = (V, E) $, where $V$ is a non-empty finite set representing the nodes in the graph, and $E$ is a finite set representing the edges between nodes. In the field of \gnids, the nodes represent machines and edges represent communication flows. Graphs are typically divided into two categories: static graphs and dynamic graphs. Static graphs are often used to represent
the steady-state structure of a network while dynamic graphs capture the evolving nature of network traffic and system interactions over time, reflecting changes in connections and activities.}

\pj{\gnids use graph encoders to generate embeddings of nodes and edges based on normal traffic data. For dynamic graphs, temporal encoders are often employed to capture graph temporal dynamics. Graph Neural Networks (GNNs) are typically used for both graph and temporal
encoders. By learning normal traffic patterns, \gnids detect any deviations as suspicious behavior. They show strong detection
performance, even against unknown attacks like zero-day exploits, and offer greater adaptability than traditional NIDS. In recent years, diverse \gnids have been proposed~\cite{yu2018netwalk, paudel2022pikachu, king2023euler, xu2024understanding, venturi2023arganids, caville2022anomal, lo2022graphsage, khoury2024jbeil, hajiramezanali2019variational}. These \gnids are summarized in Table~\ref{tab:NIDS}.}

\end{comment}  



%In particular, \pikachu leverages temporal random walk and Gate Recurrent Unit (GRU) to detect malicious communications within the network. \euler proposes a formalized framework that distributes graph convolution layers across multiple hosts to accelerate the training process. \argus takes the attributes of edges into account to minimize the false positive rate.

\begin{comment}
\begin{table*}
\centering
\caption{Comparison of SOTA \gnids. "Attr" stands for "Attributes". ''Stg'' stands for  ''Streaming'' that indicates if predictions can be performed incrementally on the ingested network traffic data.}
\label{tab:NIDS}
\scalebox{1.0}{
\begin{tabular}{c|ccccccc} 
\hline
System                                                                   & \begin{tabular}[c]{@{}c@{}}Graph\\Type\end{tabular} & Node                                                                              & Edge                                    & \begin{tabular}[c]{@{}c@{}}Graph\\Encoder\end{tabular} & \begin{tabular}[c]{@{}c@{}}Temporal \\Encoder\end{tabular} & Streaming & \begin{tabular}[c]{@{}c@{}}Open\\Source\end{tabular}  \\ 
\hline
\begin{tabular}[c]{@{}c@{}}NETWALK\\(KDD 2018)\end{tabular}              & Static                                              & \begin{tabular}[c]{@{}c@{}}\textcolor[rgb]{0.2,0.2,0.2}{\checkmark}\\\end{tabular} & \times                                   & Network walk Autoencoder                               & NO                                                         & YES       & YES                                                   \\ 
\hline
\begin{tabular}[c]{@{}c@{}}ARGA\\(ACM 2023)\end{tabular}                 & Static                                              & \textcolor[rgb]{0.2,0.2,0.2}{\checkmark}                                           & \textcolor[rgb]{0.2,0.2,0.2}{\checkmark} & GAE                                                    & NO                                                         & YES       & NO                                                    \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Anomal-E\\(KBS 2022)\end{tabular}             & Static                                              & \textcolor[rgb]{0.2,0.2,0.2}{\checkmark}                                           & \textcolor[rgb]{0.2,0.2,0.2}{\checkmark} & GraphSAGE                                              & NO                                                         & YES       & YES                                                   \\ 
\hline
\begin{tabular}[c]{@{}c@{}}E-GraphSAGE\\（NOMS 2022）\end{tabular}         & Static                                              & \textcolor[rgb]{0.2,0.2,0.2}{\checkmark}                                           & \textcolor[rgb]{0.2,0.2,0.2}{\checkmark} & GraphSAGE                                              & NO                                                         & YES       & YES                                                   \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Jbeil\\(IEEE S\&P 2024)\end{tabular}          & Dynamic                                             & \textcolor[rgb]{0.2,0.2,0.2}{\checkmark}                                           & \textcolor[rgb]{0.2,0.2,0.2}{\checkmark} & TGN                                                    & GRU                                                        & YES       & YES                                                   \\ 
\hline
\begin{tabular}[c]{@{}c@{}}VGRNN\\(NeurIPS 2019)\end{tabular}            & Dynamic                                             & \textcolor[rgb]{0.2,0.2,0.2}{\checkmark}                                           & \times                                   & GCN                                                    & GRNN                                                       & YES       & YES                                                   \\ 
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{EULER}\\(NDSS 2022)\end{tabular}            & Dynamic                                             & \textcolor[rgb]{0.2,0.2,0.2}{\checkmark}                                           & \times                                   & GNN                                                    & \begin{tabular}[c]{@{}c@{}}GRU /\\LSTM\end{tabular}        & YES       & YES                                                   \\ 
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{PIKACHU}\\(NOMS 2022)\end{tabular}                                    & Dynamic                                             & \textcolor[rgb]{0.2,0.2,0.2}{\checkmark}                                           & \times                                   & Random Walk + Skip-gram                                & GRU                                                        & NO        & YES                                                   \\ 
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{ARGUS}\\(IEEE S\&P~2024)\end{tabular} & Dynamic                                             & \textcolor[rgb]{0.2,0.2,0.2}{\checkmark}                                           & \textcolor[rgb]{0.2,0.2,0.2}{\checkmark} & MPNN                                                   & GRU                                                        & YES       & YES                                                   \\
\hline
\end{tabular}
}

\end{table*}
\end{comment}

%At a high level, NIDS can be categorized into two types: rule-based~\cite{zeek, suricata, snort, modSecurity, yara} and learning-based~\cite{yu2018netwalk, paudel2022pikachu, king2023euler, kipf2016variational, xu2024understanding}, which we explain in more detail below.

%Rule-based NIDS rely on a predefined set of rules (\eg Suricata Traffic ID ruleset) to detect network attacks. These rules describe the characteristics or behavioral patterns of suspicious behaviors. When network traffic matches one rule, NIDS triggers a corresponding alert to notify security analysts. Rule-based NIDS have multiple advantages, such as high interpretability of alerts, low false positive rates, and real-time responsiveness. However, these systems face two significant limitations: 1) They fail to identify attack patterns that are not covered in the rule set, resulting in high false negative rates. 2) It requires substantial costs to maintain the rule set, which hinders the automation of detection.

%In contrast, learning-based NIDS identify suspicious behaviors by analyzing the normal patterns of network traffic, without the need of predefined rule sets. To achieve it, NIDS first utilize normal network data to train a machine learning model. Then, they take new traffic data as input to make prediction. Any behavior that deviates from the expected patterns will be detected. Learning-based NIDS demonstrate good detection performance, even in the face of unknown attacks (\eg zero-day attacks), exhibiting greater adaptability than rule-based NIDS. With the rise of artificial intelligence technology, researchers have leveraged neural network models to build NIDS in recent years. Among SOTA works, PIKACHU~\cite{paudel2022pikachu}, EULER~\cite{king2023euler}, and ARGUS~\cite{xu2024understanding} are the most representative ones. In particular, PIKACHU leverages temporal random walk and GRU to detect malicious communications in the network. EULER proposes a formalized framework that distributes graph convolution layers across multiple hosts to accelerate the training process. ARGUS takes the attributes of edges into consideration to reduce the false positive rate. The detailed comparison of learning-based NIDS are shown in table \ref{tab:NIDS}


%\subsection{Public Evaluation Datasets}
%Traffic data is a key component to train and evaluate \gnids. Researchers primarily utilize two publicly available datasets, the LANL dataset~\cite{lanl} and DARPA OpTC~\cite{optc}, to assess the performance of SOTA \gnids. Below, we outline these datasets, whose statistical information is listed in Table~\ref{tab:dataset}.

%\textbf{LANL.} The LANL dataset is a subset of comprehensive multi-source network security event data collected by the Los Alamos National Laboratory (LANL). This dataset contains anonymized events derived from four sources: 1) authentication logs from personal computers and domain controller servers, 2) process start and stop events, 3) DNS logs from DNS servers, and 4) network traffic from routers within the internal computer network. Among these sources, authentication logs are widely used for evaluating NIDS, encompassing a total of 17,649 nodes and 1,051,430,459 events, with 299 nodes and 706 events pertaining to attacks. The entire data collection spans 58 days, during which the red team conducted multiple attacks. That said, data related to both normal user and attack behavior is collected.

%\textbf{DARPA OpTC.} The DARPA OpTC dataset is collected through the DARPA Transparent Computing (TC) program. The goal of this program is to provide high-fidelity visibility into systems and help discover modern attack activities, such as Advanced Persistent Threats (APTs). This dataset consists of host-level activities, such as processes, files, and network sockets. It includes various types of attacks stemming from adversarial actions. Over the course of 8 days, a total of 92,073,717 events were collected from 814 hosts. Among them, 28 hosts and 21,784 events are related to attacks.





